A Grounded Theory of Coordination in Remote-First and Hybrid Software Teams

While the long-term effects of the COVID-19 pandemic on software professionals and organizations are difficult to predict, it seems likely that working from home, remote-first teams, distributed teams, and hybrid (part-remote/part-office) teams will be more common. It is therefore important to investigate the challenges that software teams and organizations face with new remote and hybrid work. Consequently, this paper reports a year-long, participant-observation, constructivist grounded theory study investigating the impact of working from home on software development. This study resulted in a theory of software team coordination. Briefly, shifting from in-office to at-home work fundamentally altered coordination within software teams. While group cohesion and more effective communication appear protective, coordination is undermined by distrust, parenting and communication bricolage. Poor coordination leads to numerous problems including misunderstandings, help requests, lower job satisfaction among team members, and more ill-defined tasks. These problems, in turn, reduce overall project success and prompt professionals to alter their software development processes (in this case, from Scrum to Kanban). Our findings suggest that software organizations with many remote employees can improve performance by encouraging greater engagement within teams and supporting employees with family and childcare responsibilities.

==> Sean.tex <==
The article titled "Formulation and Preliminary Test of an Empirical Theory of Coordination in Software Engineering" \cite{herbsleb2003formulation} creates an empirical theory of coordination, and 


Herbsleb's theory: 
    finite set of engineering decisions
    
    software project is a combination of those decisions as defined by that particular project
    
    eng. decisions often have mutual constraints, so the problem of coordination is understanding, recognizing and correctly acting upon such mutual constraints as work proceeds 
    
    Feasible choices for mutually constraining decisions (i.e. solutions to coordination issues) are more likely to be made when they are made by people in frequent communication with each other
    
Our theory:
    coordination depends on factors that are usually present before the actual problems appear
    
    software team coordination in the context of remote work depends on group cohesion, trust, communication and family responsibilities.
    
    
Similarities:
    Both theories highlight the need for frequent and effective communication
    
Differences:
    It sounds like Herbsleb's idea of "problems" is more black and white. Herbsleb talks about "effects of infeasible decisions" (problems) in terms of either a failed project, defects, faults, errors or rework and its associated costs... 
    Our work talks more about effects on team members 
    
\pr{that's enough, please move on to more papers.}


The article "Global Software Engineering: The Future of Socio-technical Coordination" \cite{herbsleb2007global} talks about coordination over distance. Problems related to GSD are: absence of colocation decreases speed and efficiency, less communication and less effective communication, lack of awareness/context, incompatibilities which may be both informal and formal (i.e. culture, language, etc.) The paper goes on to discuss 4 research areas on the topic of GSD and coordination, namely; software architecture, eliciting/communicating requirements, environments and tools, orchestrating global development.


the article titled "Collaboration in software engineering projects: A theory of coordination" \cite{herbsleb2006collaboration} defines coordination theory as a DCSP (distributed constraint satisfaction problem). The factors that influence the DCSP are: geographic distribution of developers, organizational structure, social networks among developers, organizational culture that impacts communication and how constraints are discovered and handled, business influences that dictate tradeoffs, and tool infrastructure. 
